Gunrock 2.0: A User Adaptive Social Conversational System

Gunrock 2.0 is built on top of Gunrock with an emphasis on user adaptation. Gunrock 2.0 combines various neural natural language understanding modules, including named entity detection, linking, and dialog act prediction, to improve user understanding. Its dialog management is a hierarchical model that handles various topics, such as movies, music, and sports. The system-level dialog manager can handle question detection, acknowledgment, error handling, and additional functions, making downstream modules much easier to design and implement. The dialog manager also adapts its topic selection to accommodate different users' profile information, such as inferred gender and personality. The generation model is a mix of templates and neural generation models. Gunrock 2.0 is able to achieve an average rating of 3.73 at its latest build from May 29th to June 4th.

==> data_analysis.tex <==
\section{Data Analysis}
In order to better utilize live feedbacks from users,  our system also employs an automatic feedback and analysis system. The analytics system include a summary of user ratings calculaed by by conversation, and by conversation turn respectively.  In doing so, we can monitor the overall quality of our chatbots and the performance pertaining to each individual modules. Live feedback are crucial to the chatbot development that allows us to assess the quality of new features.


==> entitydetectionlinking.tex <==
\section{Entity Detection Linking} \label{sec:entity_detection_linking}


==> future_work.tex <==
\section{Future Work} \label{sec:future}

Due to the intensity and time limit of the competition, we were not able to perform rigorous experimental analysis on the innovative features of Gunrock 2.0 including but not limited to user adaptive dialog manager, acknowledgement generation and follow-up question generation. We will conduct the A/B testing right after the end of the semi-finals.

==> nlu/asr_correction.tex <==
\subsubsection{ASR Correction} \label{sssec:asr_correction}
\todo{@Dian and @Minh}

ASR error has a huge impact on NLU quality. ASK provides an overall ASR confidence score by incorporating both the confidence score for each word and the score generated by a language model. The overall score indicates how likely the whole utterance is recognized correctly. However, there are two types of false positives that may trigger error handling signaling ASR errors when the confidence score is low. The first one is when the word mentioned is not frequently seen in the training data, so the word receives a low weight. Another instance of a false positive is with homophone words that the ASR cannot capture even if the user repeats their request. %To solve these problems, we experimented with a spell checking method which does not work well due to both training data and different use cases.



We used the double metaphone algorithm \cite{dmetaphone} to compare the noun phrases (ignoring the most frequent stopwords) mentioned by the user and a knowledge base. The knowledge base includes both the context and the domain (e.g. sports genres, movies titles and game names). We stored the primary and the secondary code of the double metaphone for each word as a key with the word as the value. We also added a tertiary code to words with certain patterns based on observations (e.g.. the word ``jalapeno'' will have a tertiary code ``\code{HLPN}'' in addition to ``\code{JLPN}'' and ``\code{ALPN}''). If the overall confidence from ASR is below a threshold (set to $0.4$), we propose a candidate by matching the metaphone code of the noun phrases to that of the knowledge base. For example, we propose the topic ``obscure holidays'' and in the next turn we receive the ASR input from the user requests, ``let's talk about secure holiday''. The primary code for ``secure holiday'' is ``\code{SKRLT}'' and the primary code for ``obscure holidays'' is ``\code{APSKRLTS}''. Since it is very likely that the ASR does not detect the beginning or the ending of a phrase, we know that this might be a map with relatively high confidence. Another example is ``let's talk about the sport high ally'' received from ASR. Because we know the context of sports, we map the code of ``high ally'' to the code of ``\code{jai alai}'' in the knowledge base (sports list).



==> nlu/coreference.tex <==
\subsubsection{Coreference Resolution} \label{sssec:coreference}
\todo{@Dian}

The state-of-the-art models by Stanford CoreNLP and NeuralCoref~\footnote{\url{https://github.com/huggingface/neuralcoref}} are trained on non-conversational data and do not work well for dialog conversations in anaphora resolution. By analyzing the data gathered (2 July - 9 July), we labeled words such as ``more'' and ``one'' to undergo coreference. We replace such words by considering both the user utterance and the system response. Specifically, we store noun phrases from the request and the NERs with the detailed description from the system response into user attributes. Depending on what the user refers to (ex. person or event, male or female), we provide the corresponding coreference solution. Depending on the request, we give priorities to noun phrases from the user and NER from our response respectively.

==> nlu/topic_detection.tex <==
\subsubsection{Topic Detection} \label{sssec:topic_tection}
\todo{@Yu}
